Evaluating Neural Radiance Fields (NeRFs) for 3D Plant Geometry Reconstruction in Field Conditions

We evaluate different Neural Radiance Fields (NeRFs) techniques for the 3D reconstruction of plants in varied environments, from indoor settings to outdoor fields. Traditional methods usually fail to capture the complex geometric details of plants, which is crucial for phenotyping and breeding studies. We evaluate the reconstruction fidelity of NeRFs in three scenarios with increasing complexity and compare the results with the point cloud obtained using LiDAR as ground truth. In the most realistic field scenario, the NeRF models achieve a 74.6% F1 score after 30 minutes of training on the GPU, highlighting the efficacy of NeRFs for 3D reconstruction in challenging environments. Additionally, we propose an early stopping technique for NeRF training that almost halves the training time while achieving only a reduction of 7.4% in the average F1 score. This optimization process significantly enhances the speed and efficiency of 3D reconstruction using NeRFs. Our findings demonstrate the potential of NeRFs in detailed and realistic 3D plant reconstruction and suggest practical approaches for enhancing the speed and efficiency of NeRFs in the 3D reconstruction process.

==> Old/Extra.tex <==
\subsection{Leveraging LPIPS in Early Stopping Optimize F1 Score and Training Time}
In training NeRFs for plant scene reconstruction, the F1 score is essential for validating the accuracy of the reconstructed pointcloud against the ground truth, a step crucial for its application in precision agriculture and botanical research. The inherent challenge during the training phase of NeRFs for novel scenes is the absence of ground truth, which is paradoxically the output we aim to approximate. Moreover, the training process for NeRFs is notoriously resource-intensive, both in terms of computational load and temporal expenditure. When scaled to multiple scenes or across extensive agricultural fields, the cumulative costs become formidable.

The significant negative correlation coefficients between LPIPS and the F1 score (-0.82), PSNR (-0.81), and SSIM (-0.69) underscore the substantial impact of LPIPS on the quality of 3D reconstruction, as provided in \ref{fig:correlation_matrix}. The high magnitude of these coefficients, particularly the -0.82 with the F1 score, indicates that LPIPS is a robust predictor of reconstruction accuracy: as the perceptual similarity measure improves (meaning LPIPS decreases), the fidelity of the reconstructed pointcloud to the ground truth improves correspondingly. This is a pivotal observation, as it not only suggests the utility of LPIPS as a stand-in metric when the ground truth is unavailable but also highlights its potential as a more influential factor than traditional metrics like PSNR(0.58) and SSIM(0.37) in determining the overall quality of NeRF-generated reconstructions.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\linewidth]{material/analysis/correlation_matrix.pdf}
    \caption{Correlation Matrix among Metrics}
    \label{fig:correlation_matrix}
\end{figure}


Given this strong correlation, LPIPS emerges as a promising surrogate metric for early stopping during NeRF training. By monitoring LPIPS, one can infer the likely F1 score and make informed decisions about halting the training process. This method could substantially decrease computational costs and time, as one need not await the completion of full training to predict its efficacy in terms of F1 score. 


To further solidify the potential of LPIPS for early stopping, let's delve into Figure \ref{fig:correlation_scatter}, which showcases the scatter plots of PSNR, SSIM, and LPIPS scores against the F1 score, alongside their respective Pearson correlation coefficients prominently displayed. This visualization serves a dual purpose: first, it offers an immediate visual assessment of the relationships between these metrics, and second, it allows for a nuanced understanding of how accurately each metric predicts the true F1 score.
The exceptionally strong negative correlation between LPIPS and F1 score (-0.82) stands out. This reinforces the notion that LPIPS effectively captures the perceptual similarity between the reconstructed and ground truth point clouds, making it a reliable proxy for F1 score, the ultimate measure of reconstruction fidelity.





\begin{figure}[t!]
    \centering

    % Create a minipage for the Y-axis title
    \begin{minipage}[c]{0.03\textwidth}
        \rotatebox{90}{Value}
    \end{minipage}%
    % Create a minipage for the subfigures
    \begin{minipage}[c]{0.96\textwidth}
        \begin{subfigure}{0.3\textwidth}
            \centering
            \caption{PSNR}
            \includegraphics[width=\linewidth]{material/analysis/correlation_scatter/PSNR.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.3\textwidth}
            \centering
            \caption{SSIM}
            \includegraphics[width=\linewidth]{material/analysis/correlation_scatter/SSIM.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.3\textwidth}
            \centering
            \caption{LPIPS}
            \includegraphics[width=\linewidth]{material/analysis/correlation_scatter/LPIPS.pdf}
        \end{subfigure}
    \end{minipage}

    \vspace{1ex}
    F1 Score

    \caption{Correlation Analysis (via Pearson Coefficients): PSNR, SSIM, LPIPS vs F1 Score}
    \label{fig:correlation_scatter}
\end{figure}


\paragraph{Mathematical Explanation of LPIPS \cite{zhang2018unreasonable}:}
To quantify the perceptual differences between two image patches, \( x \) and \( x_0 \), the Learned Perceptual Image Patch Similarity (LPIPS) framework employs activations from a neural network \( F \). Features are extracted from \( L \) layers and normalized across the channel dimension. For each layer \( l \), the normalized features are represented by \( \hat{y}^l \) and \( \hat{y}^{l0} \), which exist in the space \( \mathbb{R}^{H_l \times W_l \times C_l} \). These are then weighted channel-wise by a vector \( w_l \in \mathbb{R}^{C_l} \). The perceptual distance is computed using the \( \ell_2 \) norm, both spatially and across channels, as expressed in the equation:

\begin{equation}
d(x, x_0) = \sum_{l} \frac{1}{H_l W_l} \sum_{h,w} \left\| w_l \odot (\hat{y}^l_{hw} - \hat{y}^{l0}_{hw}) \right\|_2^2
\end{equation}

This distance metric, \( d(x, x_0) \), provides a scalar value indicating the perceptual dissimilarity between the patches. The vector \( w_l \) weights the contribution of each channel to the distance metric. By setting \( w_l \) to \( 1/\sqrt{C_l} \), the computation effectively measures the cosine distance, highlighting the directional alignment of the feature vectors instead of their magnitude.


\paragraph{Algorithm for Plateau Detection Incorporating LPIPS:}
The plateau detection algorithm identifies a stabilization point in a series of metric values, such as LPIPS. 

\begin{algorithm}
\caption{Plateau Detection Algorithm with LPIPS}
\begin{algorithmic}[1]
\Procedure{DetectPlateau}{$\mathcal{S}, \mathcal{G}, \theta, C$} \Comment{Inputs: Sets of images per iteration $\mathcal{S}$, Sets of GT images $\mathcal{G}$, threshold $\theta$, consistency length $C$}
    \State Initialize an empty list $\mathcal{M}$ to store average LPIPS values over training iterations.
    \For{each set $\mathcal{I}$ and corresponding GT set $\mathcal{G}_I$ in $\mathcal{S}$ and $\mathcal{G}$}
        \State Initialize $\text{sumLPIPS} = 0$.
        \For{each image $I$ and corresponding GT image $G$ in $\mathcal{I}$ and $\mathcal{G}_I$}
            \State $\text{sumLPIPS}$ += $\text{LPIPS}(I, G)$.
        \EndFor
        \State Compute average LPIPS for the set: $\text{avgLPIPS} = \text{sumLPIPS} / |\mathcal{I}|$.
        \State Append $\text{avgLPIPS}$ to $\mathcal{M}$.
    \EndFor
    \If{$|\mathcal{M}| < C$}
        \State \Return $0$ \Comment{Insufficient data for plateau detection}
    \EndIf
    \For{$i = 1$ to $|\mathcal{M}| - 1$}
        \State Let $\text{consistent} = \text{True}$.
        \For{$j = \max(0, i - C + 1)$ to $i$}
            \If{$|\mathcal{M}[j] - \mathcal{M}[j - 1]| \geq \theta$}
                \State Set $\text{consistent} = \text{False}$ and \textbf{break}.
            \EndIf
        \EndFor
        \If{$\text{consistent}$}
            \State \Return $i$ \Comment{Plateau point detected, Output: $P$}
        \EndIf
    \EndFor
    \State \Return $|\mathcal{M}| - 1$ \Comment{No plateau detected, Output: $P$}
\EndProcedure
\end{algorithmic}
\end{algorithm}


The updated algorithm computes the average Learned Perceptual Image Patch Similarity (LPIPS) for each set of images in \(\mathcal{S}\) against their corresponding ground truth images in \(\mathcal{G}\). It then assesses the sequence of these average LPIPS values to identify a plateau, using a specified threshold \(\theta\) and a consistency length \(C\). The detection of the plateau point \(P\) is crucial for indicating an optimal stopping point in the training process.



\paragraph{Results: } The implementation of early stopping based on the LP-IPS metric yielded substantial savings in computational time across all scenarios, with a minor sacrifice in the fidelity of 3D reconstructions, as measured by the F1 score. As illustrated in Figure \ref{fig:lpips_vs_f1}, the time savings were notable across the three tested methodologies—Instant-NGP, TensorRF, and NeRFacto—with each showing a marked decrease in training time without a commensurate loss in F1 score accuracy.

On average, the early stopping strategy resulted in a 61.1\% reduction in training time, suggesting a significant efficiency gain in the process of 3D plant reconstruction using neural radiance fields. Concurrently, the average F1 score loss was contained to 7.4\%, indicating that the early plateau detection has a moderate impact on the quality of the 3D point cloud reconstructions.






\begin{figure}[t!]
    \centering

    % Y-axis title for the first set of subfigures
    \begin{minipage}[c]{0.03\textwidth}
        % \rotatebox{90}{\centering Score}
    \end{minipage}%
    \begin{minipage}[c]{0.96\textwidth}
        \begin{subfigure}{0.3\textwidth}
            \centering
            \caption{Instant-NGP (Scene-I)}
            \includegraphics[width=\linewidth]{material/analysis/lpips_vs_f1/Instant-NGP_scenario1.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.3\textwidth}
            \centering
            \caption{TensoRF (Scene-I)}
            \includegraphics[width=\linewidth]{material/analysis/lpips_vs_f1/TensoRF_scenario1.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.3\textwidth}
            \centering
            \caption{NeRFacto (Scene-I)}
            \includegraphics[width=\linewidth]{material/analysis/lpips_vs_f1/NeRFacto_scenario1.pdf}
        \end{subfigure}
    \end{minipage}

    % Y-axis title for the second set of subfigures
    \begin{minipage}[c]{0.03\textwidth}
        % \rotatebox{90}{\centering Score}
    \end{minipage}%
    \begin{minipage}[c]{0.96\textwidth}
        \begin{subfigure}{0.3\textwidth}
            \centering
            \caption{Instant-NGP (Scene-II)}
            \includegraphics[width=\linewidth]{material/analysis/lpips_vs_f1/Instant-NGP_scenario2.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.3\textwidth}
            \centering
            \caption{TensoRF (Scene-II)}
            \includegraphics[width=\linewidth]{material/analysis/lpips_vs_f1/TensoRF_scenario2.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.3\textwidth}
            \centering
            \caption{NeRFacto (Scene-II)}
            \includegraphics[width=\linewidth]{material/analysis/lpips_vs_f1/NeRFacto_scenario2.pdf}
        \end{subfigure}
    \end{minipage}
    
    % Y-axis title for the second set of subfigures
    \begin{minipage}[c]{0.03\textwidth}
        % \rotatebox{90}{\centering Score}
    \end{minipage}%
    \begin{minipage}[c]{0.96\textwidth}
        \begin{subfigure}{0.3\textwidth}
            \centering
            \caption{Instant-NGP (Scene-III)}
            \includegraphics[width=\linewidth]{material/analysis/lpips_vs_f1/Instant-NGP_scenario3.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.3\textwidth}
            \centering
            \caption{TensoRF (Scene-III)}
            \includegraphics[width=\linewidth]{material/analysis/lpips_vs_f1/TensoRF_scenario3.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.3\textwidth}
            \centering
            \caption{NeRFacto (Scene-III)}
            \includegraphics[width=\linewidth]{material/analysis/lpips_vs_f1/NeRFacto_scenario3.pdf}
        \end{subfigure}
    \end{minipage}
    \vspace{1ex}
    Number of Iterations

    % Shared Legend
    \vspace{1ex}
    \raisebox{0ex}{\textcolor{red}{\rule[0.5ex]{0.1cm}{1pt}\hspace{0.1cm}\rule[0.5ex]{0.1cm}{1pt}\hspace{0.1cm}\rule[0.5ex]{0.1cm}{1pt}}} Detected Plateau Point \quad
    \raisebox{0.5ex}{\textcolor{blue}{\rule{0.5cm}{1pt}}} LPIPS \quad
    \raisebox{0.5ex}{\textcolor{green}{\rule{0.5cm}{1pt}}} F1 Score \quad
    \textcolor{black}{\textbullet} Original \quad
    \textcolor{black}{$\times$} Interpolated \quad

    \caption{Early Stopping Based on LPIPS}
    \label{fig:lpips_vs_f1}
\end{figure}

Specifically, Instant-NGP presented a more pronounced variation in F1 score loss, which was notably higher in Scene-III, thereby affecting its average loss more significantly than TensorRF and NeRFacto. TensorRF and NeRFacto showed a remarkable consistency in time savings, which was mirrored in their comparable F1 score losses, highlighting the robustness of these methods in early stopping scenarios.

These findings articulate a compelling case for the utilization of early stopping in NeRF-based 3D reconstruction tasks, emphasizing the need to balance between computational resources and reconstruction precision. Such a balance is pivotal in scenarios where time efficiency is paramount yet a minimal compromise on reconstruction accuracy is permissible.



